Responsible and Inclusive Technology Framework: A Formative Framework to Promote Societal Considerations in Information Technology Contexts

Technology development practices in industry are often primarily focused on business results, which risks creating unbalanced power relations between corporate interests and the needs or concerns of people who are affected by technology implementation and use. These practices, and their associated cultural norms, may result in uses of technology that have direct, indirect, short-term, and even long-term negative effects on groups of people and/or the environment. This paper contributes a formative framework -- the Responsible and Inclusive Technology Framework -- that orients critical reflection around the social contexts of technology creation and use; the power dynamics between self, business, and societal stakeholders; the impacts of technology on various communities across past, present, and future dimensions; and the practical decisions that imbue technological artifacts with cultural values. We expect that the implementation of the Responsible and Inclusive Technology framework, especially in business-to-business industry settings, will serve as a catalyst for more intentional and socially-grounded practices, thus bridging the responsibility and principles-to-practice gap.

==> Tables/table_1.tex <==

% \newpage

% \begin{landscape}

% \begin{table}[hb!]
%   \footnotesize
%   \centering
%   \begin{tabular}{p{3cm} p{10cm} p{2.5cm} p{1.5cm}}
%     % \toprule
%     {\small\textit{Framework}} & {\small \textit{Dimensions/components}} & Domain & Originating organization from\\
%     \midrule   
% 	Responsible Chain Management~\cite{Bakker2002} & Interpretations of stakeholder interests, integration into business processes, monitoring these processes, and communication with stakeholders. & Supply chain & Netherlands \\ \hline
%     Responsible Innovation~\cite{Stilgoe2013} & Anticipation, reflexivity, inclusion, and responsiveness. & Geoengineering & UK \\ \hline
%     Responsible Innovation in Health~\cite{Pacifico2018} & Population health, health system, economic, organizational and environmental & Healthcare & Canada \\ \hline
%     Inclusive and Adaptive Framework~\cite{Saja2018} & Social structure, social capital, social mechanisms, social equity, and social belief. & Natural disasters & Sri Lanka \\ \hline
%     Unified Framework of Five Principles for AI in Society~\cite{Floridi2019} & Beneficence, non-maleficence, autonomy, justice, and explicability. & Responsible AI & US \\ \hline
%     Suresh and Guttag's framework~\cite{Suresh2019} & Historical bias, representation bias, measurement bias, aggregation bias, learning bias, evaluation bias, and deployment bias. & Responsible AI & US \\ \hline    
%     Impact Assessment Framework~\cite{Schiff2020} & Broad, operationalizable, flexible, iterative, guided, and participatory. & Responsible AI & US \\ \hline
%     AIRR~\cite{Ludwig2020} & Anticipation, inclusion, reflexivity, and responsiveness. & Traditional ecological knowledge & Europe \\ \hline
%     Choices Framework~\cite{Benjamins2021} & Bias, explainability, agency, errors, continuous autonomous learning, privacy, security, and safety. & Responsible AI & Europe \\ \hline
%     Feminist Data Ethics of Care Framework~\cite{Gray2021} & Ensuring diverse representation and participation in the ML economy, critically evaluating positionality, centering human subjects at every stage of the ML pipeline, implementing transparency and accountability measures, and  equitably distributing the responsibility for operationalizing a feminist data ethics of care praxis. & Responsible AI & Australia \\ \hline
%     Deliberative Framework for AI Governance~\cite{Buhmann2021} & corporation, media, and civil society. & Responsible AI & Europe \\ \hline
%     Shneiderman's Recommendations \cite{Shneiderman2021} & Audit trails and analysis tools, software engineering workflows, verification and validation testing, bias testing to enhance fairness, explainable user interfaces, leadership commitment to safety, hiring and training oriented to safety, extensive reporting of failures and near misses, internal review boards for problems and future plans, alignment with industry standard practices, government interventions and regulation, accounting firms conduct external audits for AI systems, insurance companies compensate for AI failures, non-governmental and civil society organizations, and professional organizations and research institutes. & Responsible AI \& UX Design & US \\ \hline
%     Dataset Deprecation Framework~\cite{Luccioni2022} & Deprecation report, system of permanent identifiers, and centralized repository for managing deprecation. & Data management & US \\ \hline
%     Licensing as a legal framework~\cite{Contractor2022} & Licensor, licensee, identification of the subject intellectual property, and restrictions. & Responsible AI & US \\ \hline
%     MATCH~\cite{Liao2022} & The underlying model attributes, system affordances to communicate AI trustworthiness cues, and users’ cognitive processing of these cues by invoking trust-related heuristics. & Responsible AI & US \\ \hline
%     Goetze's Framework~\cite{Goetze2022} & Vicarious responsibility and moral entanglement & Autonomous Systems & US \\ \hline
%     Workshop Framework \cite{Klumbyte2022} & Situated knowledges, Figurations, Diffraction, and Critical Fabulation/Speculation. & Speculative Design in AI & Germany \\ \hline
%     Sloane and Zakrzewski's framework~\cite{Sloane2022} & Practice based on technical and socio-technical innovation. & Responsible AI & Germany \\ \hline
%     % \bottomrule
%   \end{tabular}
%   \caption{Summary of frameworks and principles covered in the literature.}~\label{tab:frameworks}
% \end{table}

% \end{landscape}
